A framework for modelling Molecular Interaction Maps

Metabolic networks, formed by a series of metabolic pathways, are made of intracellular and extracellular reactions that determine the biochemical properties of a cell, and by a set of interactions that guide and regulate the activity of these reactions. Most of these pathways are formed by an intricate and complex network of chain reactions, and can be represented in a human readable form using graphs which describe the cell cycle checkpoint pathways. This paper proposes a method to represent Molecular Interaction Maps (graphical representations of complex metabolic networks) in Linear Temporal Logic. The logical representation of such networks allows one to reason about them, in order to check, for instance, whether a graph satisfies a given property $\phi$, as well as to find out which initial conditons would guarantee $\phi$, or else how can the the graph be updated in order to satisfy $\phi$. Both the translation and resolution methods have been implemented in a tool capable of addressing such questions thanks to a reduction to propositional logic which allows exploiting classical SAT solvers.

==> literature.tex <==

\section{Logical Approaches to Biological Systems}
\label{approaches}

The typical objects to be modelled in the framework of Systems Biology are
\emph{networks} of interacting elements that evolve in time. According
to the features of the network and its properties, various approaches
can be followed,  which can   describe the dynamics of the
system taking the following elements into consideration: 
\begin{itemize}
	\item \textbf{Components}: they are represented by variables,
          which can be either \emph{discrete} or \emph{continuous} depending
          on the requirements of the model. 
	\item \textbf{Interactions}: they are represented by rules
          that specify the dynamical changes of the variables. These
          interactions can  in  turn be classified according to
 the adopted representation of  time  (\emph{discrete} or
 \emph{continuous}). Finally, the execution of an action can be either
 \emph{stochastic} or not, if a certain degree of
 uncertainty is considered, reflecting the assumption of a noisy environment. 
\end{itemize}

According to these possible semantics, the various modelling
approaches may be classified as follows~\cite{FH07}:  

\begin{itemize}
	\item Models involving continous component quantities and
          deterministic interactions: these models are mathematical,
          inherently quantitative and usually based on ordinary
          differential equations. Tools like Timed Automata
          representations or Continuous-Time Markov Chains are used in
          the construction of models of this category. 
	\item Discrete-value models: they are characterised by the use
          of discrete time. Approaches like executable models based on
          Finite State Machines representations or stochastic models
          such as Discrete-Time Markov Chains belong to this
          category. 
\end{itemize}

\noindent Other hybrid models such as Hybrid Automata or Process
Algebraic Techniques, mix discrete and continuous representation for
both variables and time dynamics. Regarding biological properties, we
can differentiate between \emph{qualitative} and \emph{quantitative}:
in the former type, time has an implicit consideration while the
latter involves reasoning on the dynamics of the system along time. To
give an example, \emph{reachability} and  \emph{temporal ordering of
  events} are considered qualitative properties while
\emph{equilibrium states} and \emph{matabolite} dynamics are
quantitative properties.  


Gene Regulatory Networks (GRNs) have been very well studied in the
temporal context because the interaction between components may be
easily represented by their presence/absence, i.e components are
represented by  boolean variables and  interactions are represented by
logical rules on their values. Following this approach Chabrier et
al.~\cite{CC+04} successfully modeled a very large network, involving
more than 500 genes. They defined  Concurrent Transition Systems
(CTS), a modelling syntax that permits to define modular systems, and
is after translated in the NuSMV language. They checked using CTL
reachability, stability and temporal ordering properties. A similar
study on a much smaller (although real) biological system has been
performed in~\cite{BM11}. Here  the LTL specification
syntax and the Spin model checker are used to verify stability properties. 

When a quantitative approach is chosen, the model dimensions drop
drastically. This is essentially due to lack of knowledge on the
parameter values for all the interactions, and 
to the increased computational complexity deriving from a large
model. In this kind of settings logic has been used to verify temporal
properties on the representations. For instance,
\cite{BRJ+05,Fages04,F08}  use CTL to verify, among other
properties, reachability and stability on different types of
biological networks, and in ~\cite{Brim13} such properties are
checked by using LTL. All these approaches are supported not only for
theoretical results but also for tools and frameworks that allow
biologists to describe a biological network and then verify whether
such representations satisfy some desired properties. Among others,
the systems BIOCHAM~\cite{CFS06}, Bio-PEPA~\cite{C08,PP13} and
ANIMO~\cite{Scholma14} are very popular in the community. 

Some
considerations can be made from the study of the aforementioned
contributions: 

\begin{itemize}
	\item the size of the modelled systems is generally very
          small, and a great degree of abstraction and suitable tools
          are needed to deal with large models; 
	\item qualitative approaches are generally enough to analyse a
          large variety of interesting biological properties; 
	\item temporal logic plays an important role in the representation and verification of biological systems.
\end{itemize}

Contrarily to approaches incorporating quantitative information into the
temporal formalisation~\cite{chabrier04}, our contribution belongs to
the category of 
qualitative approaches, since quantitative information in biological
relations, such as the quantity of reactives and their speed of consumption
in a reaction, are not formalised. We are mostly interested in
formalising the interaction among the different components of the
system and how they evolve in time according to the different reactions.  
	 

